Surface and bulk critical behaviour of the XY chain in a transverse field

The surface magnetization of the quantum XY chain in a transverse field is found for arbitrary nearest neighbour interactions in closed form. This allows to derive the bulk phase diagram in a simple way. The magnetic surface behaviour and the bulk correlation length are found exactly.

==> xref.tex <==
\catcode`@=11 
\newwrite\auxfile 
\newwrite\xreffile 
\newif\ifxrefwarning \xrefwarningtrue 
\newif\ifauxfile 
\newif\ifxreffile 
\def\testforxref{\begingroup 
    \immediate\openin\xreffile = \jobname.xrf\space 
    \ifeof\xreffile\global\xreffilefalse 
    \else\global\xreffiletrue\fi 
    \immediate\closein\xreffile 
    \endgroup} 
\def\testforaux{\begingroup 
    \immediate\openin\auxfile = \jobname.aux\space 
    \ifeof\auxfile\global\auxfilefalse 
    \else\global\auxfiletrue\fi 
    \immediate\closein\auxfile 
    \endgroup} 
\def\openreffile{\immediate\openout\auxfile = \jobname.aux}% 
\def\readreffile{% 
    \testforxref 
    \testforaux 
    \ifxreffile 
       \begingroup 
         \@setletters 
         \input \jobname.xrf 
       \endgroup 
    \else 
\message{No cross-reference file existed, some labels may be undefined}% 
    \fi\openreffile}% 
\def\@setletters{% 
    \catcode`_=11 \catcode`+=11 
    \catcode`-=11 \catcode`@=11 
    \catcode`0=11 \catcode`1=11 
    \catcode`2=11 \catcode`3=11 
    \catcode`4=11 \catcode`5=11 
    \catcode`6=11 \catcode`7=11 
    \catcode`8=11 \catcode`9=11 
    \catcode`(=11 \catcode`)=11 
    \catcode`:=11 \catcode`'=11 
    \catcode`&=11 \catcode`;=11 
    \catcode`.=11}% 
\gdef\el@b{\eqlabel} 
\gdef\sl@b{\seclabel} 
\gdef\tl@b{\tablabel} 
\gdef\fl@b{\figlabel} 
\def\l@belno{\ifx\labeltype\el@b  
   \let\labelno=\en\def\@label{\eqlabel}%  
   \else\let\labelno=\ignorespaces 
   \ifx\labeltype\sl@b \def\@label{\seclabel}% 
   \else\ifx\labeltype\tl@b \def\@label{\tablabel}%  
   \else\ifx\labeltype\fl@b \def\@label{\figlabel}% 
   \else\def\@label{\seclabel}\fi\fi\fi\fi} 
\def\label#1{\l@belno\expandafter\xdef\csname #1@\endcsname{\@label}% 
    \immediate\write\auxfile{\string 
    \gdef\expandafter\string\csname @#1\endcsname{\@label}}% 
    \labelno}% 
\def\ref#1{% 
    \expandafter \ifx \csname @#1\endcsname\relax 
    \message{Undefined label `#1'.}% 
    \expandafter\xdef\csname @#1\endcsname{(??)}\fi  
    \csname @#1\endcsname}% 
\readreffile 
% 
%%%%%%%%%%% 
% 
\def\bibitem#1{\global\advance\refno by 1% 
    \immediate\write\auxfile{\string 
    \gdef\expandafter\string\csname #1@\endcsname{\the\refno}}% 
    \rf{[\the\refno]}}% 
\def\bitem[#1]#2{\immediate\write\auxfile{\string 
    \gdef\expandafter\string\csname #2@\endcsname{#1}}% 
    \rf{[#1]}}% 
% 
\def\cite#1{\hbox{[\splitarg{#1}]}}% 
\def\splitarg#1{\@pt#1,\@ptend}% 
\def\@pt#1,#2\@ptend{\ifempty{#1}\else 
    \@pttwo #1\@pttwoend 
    \ifempty{#2}\else\sp@cer\@pt#2\@ptend\fi\fi}% 
\def\@pttwo#1\@pttwoend{\expandafter 
    \ifx \csname#1@\endcsname\@pttwoend\else 
    \@ifundefined{#1}{{\bf ?}% 
    \message{Undefined citation `#1' on page  
    \the\pageno}}{\csname#1@\endcsname}\fi}% 
\def\@pttwoend{@@@@@}% 
\def\sp@cer{,\nobreak\thinspace}% 
\def\ifempty#1{\@ifempty #1\@xx\@xxx}% 
\def\@ifempty#1#2\@xxx{\ifx #1\@xx}% 
\def\@xx{@@@@}% 
\def\@xxx{@@@@}% 
\long\def\@ifundefined#1#2#3{\expandafter\ifx\csname 
  #1@\endcsname\relax#2\else#3\fi}% 
% 
\catcode`@=12 
\endinput 
 
% 28/10/93 Added \bitem definition for non numeric cross referencing  

